First On-Orbit Demonstration of a Geospatial Foundation Model

Geospatial foundation models (GeoFMs) promise broad generalisation capacity for Earth observation (EO) tasks, particularly under data-limited conditions. However, their large size poses a barrier to deployment on resource-constrained space hardware. To address this, we present compact variants of a Vision Transformer (ViT)-based GeoFM that preserve downstream task performance while enabling onboard execution. Evaluation across five downstream tasks and validation in two representative flight environments show that model compression and domain adaptation are critical to reducing size and resource demands while maintaining high performance under operational conditions. We further demonstrate reliable on-orbit inference with the IMAGIN-e payload aboard the International Space Station. These results establish a pathway from large GeoFMs to flight-ready, resource-efficient deployments, expanding the feasibility of onboard AI for EO missions.

==> MISC/NOTES.tex <==
Example - https://www.nature.com/articles/s42256-025-01026-6

https://www.nature.com/natmachintell/submission-guidelines




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Aims & Scope - https://www.nature.com/natmachintell/aims
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Nature Machine Intelligence publishes high-quality original research and reviews in a wide range of topics in machine learning, robotics and AI.  We also explore and discuss the significant impact that these fields have on other scientific disciplines as well as many aspects of society and industry. There are countless opportunities where machine intelligence can enhance human capabilities and knowledge in fields such as scientific discovery, healthcare, medical diagnostics and safe and sustainable cities, transport and agriculture. At the same time, many important questions on ethical, social and legal issues arise, especially given the fast pace of developments. Nature Machine Intelligence provides a platform to discuss these wide implications — encouraging a cross-disciplinary dialogue — with Comments, News Features, News & Views articles and also Correspondence.

Like all Nature-branded journals, Nature Machine Intelligence is run by a team of professional editors and dedicated to a fair and rigorous peer-review process, high standards of copy-editing and production, swift publication, and editorial independence.

Disciplines covered in the journal
AI, robotics, AI and cognitive science, human-robot interaction, machine learning, deep learning, reinforcement learning, robot learning, artificial neural networks, symbolic reasoning, computer vision, natural language processing, genetic and evolutionary computing, neuro-inspired computing, humanoid robots, swarm robotics, bio-inspired robotics, soft robotics, multi-agent systems and so on.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Content types - https://www.nature.com/natmachintell/content
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

An Article is a substantial novel research study, with a complex story often involving several techniques or approaches. 

Format:

Main text (introduction, results, discussion) – up to 3,500 words, excluding abstract, Methods, references and figure legends.
Abstract – up to 150 words, unreferenced. 
Display items – up to 6 items (figures and/or tables). 
Article should be divided as follows: 
Introduction (without heading) 
Results
Discussion
Methods. 
NOTE: Results and Methods should be divided by topical subheadings; the Discussion does not contain subheadings. 
References – as a guideline, we typically recommend up to 50.
Articles include received/accepted dates. 
Articles may be accompanied by supplementary information. 
Articles are peer reviewed.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this work, we propose a practical framework for deploying and executing a ViT-based GFM onboard two EO missions: Kanyini and IMAGIN-e (Figure~\ref{fig:framework}). By combining model compression with task-specific domain adaptation, we tailor foundation models to meet the stringent power, memory, and compute constraints of space-qualified hardware while maintaining high performance under real-world conditions. Our contributions are threefold: (1) we present the first demonstration of onboard GFM deployment for EO satellite processing; (2) we adapt a method for compressing a pretrained GFM into a compact variant suitable for edge platforms; and (3) we demonstrate the real-world effectiveness of a bandwidth-efficient adaptation strategy that enables accurate and generalisable inference in orbit. This strategy also supports updates of larger and more complex models, overcoming the limitations of conventional lightweight-only deployments. We validate this framework through hardware-in-the-loop testing and evaluation on real satellite imagery acquired in orbit. While onboard demonstrations were successfully conducted on IMAGIN-e, deployment on Kanyini was validated using the HyperScout-2 engineering model - its flight-intended imaging payload - due to unforeseen technical issues with the spacecraft.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Foundation model can be compressed for onboard deployment while preserving task performance}\label{result1}
% \hl{UPDATE THIS} To enable deployment on resource-constrained satellite platforms, we developed compact GFMs by compressing Prithvi-EO-2.0-300M~\cite{szwarcman2024prithvi}, a 300M parameter ViT-based foundation model (i.e., the pretrained encoder used throughout this work) designed for EO tasks, while preserving downstream task performance. The resulting variants — Prithvi-EO-2.0-512 and Prithvi-EO-2.0-256 — have smaller patch embedding dimensions of 512 and 256, respectively, compared to 1024 in the original 300M model. This results in approximately 4× and 16× reductions in parameter count and model size. Both variants were pretrained using a dual-MAE (masked autoencoder) distillation approach, where a smaller student model learns to reconstruct the outputs of a larger, frozen teacher model. This enables the student to inherit transferable representations without relying on labelled data. Further architectural and training details are provided in Section~\ref{method1}. \\

% Following pretraining, all configurations of Prithvi-EO-2.0 were evaluated on six downstream tasks by attaching task-specific heads. These heads were fine-tuned on datasets with spatial and spectral properties similar to the target domain (i.e., data encountered during satellite deployment), while keeping the foundation model parameters frozen. Figure~\ref{fig:eo-task-results} summarises the performance across these tasks, comparing the original Prithvi-EO-2.0-300M, compact variants pretrained via MAE (512-MAE, 256-MAE), and those pretrained via dual-MAE distillation (512-MAE-D, 256-MAE-D). Across all tasks, the dual-MAE distilled variants consistently match or outperform their MAE-only counterparts, despite having significantly fewer parameters than the original model. Among the compact variants, 256-MAE-D offers the best trade-off between accuracy and efficiency. It matches or exceeds the performance of other variants in most tasks — including cloud detection, flood detection, and biomass estimation — while requiring the fewest resources, making it well-suited for onboard deployment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Foundation model supports generalisation to the target domain and reduces training data needs}\label{results2}

% We next evaluate how well the foundation model (pretrained encoder) generalises to the target domain and supports adaptation with varying amounts of labelled data. Domain adaptation was performed using imagery from the Kanyini and IMAGIN-e missions. As all Prithvi-V2-EO variants achieved comparable performance across downstream tasks, we selected the most compact and highest-performing configuration (Prithvi-EO-2.0-256-MAE-D) together with its task-specific heads for this stage. We focus here on cloud and flood detection as representative downstream tasks, excluding others due to the absence of suitable ground truth data: the dataset contained no visible landslide events; land cover classification would require prohibitively time-intensive manual annotation across 11 semantic classes; and above-ground biomass estimation depends on spatially co-located reference maps derived from field plots, airborne LiDAR, or calibrated satellite models, none of which are available for the Kanyini or IMAGIN-e scenes. \\

% As shown in Fig.~\ref{fig:training-data-results}, we evaluated the pretrained encoder (Prithvi-EO-2.0-256-MAE-D) and task-specific heads on cloud detection (classification and segmentation) and flood detection (segmentation) in the Kanyini domain, using 100\%, 50\%, and 25\% of the available labelled training data. Each experiment was repeated five times with different random seeds. We compared three configurations: (1) randomly initialised encoder and task head (no pretraining); (2) pretrained (frozen) encoder with a randomly initialised task head (pretrained encoder); and (3) pretrained (frozen) encoder with a pretrained task head (pretrained encoder + head). Error bars indicate the standard deviation across runs. Pretrained models consistently outperformed models trained from scratch when the labelled dataset was reduced to 50\% or 25\%, indicating that the pretrained encoder substantially reduces the amount of labelled data required while preserving strong downstream performance. With the full training set, the pretrained encoder matched or exceeded the performance of models trained from scratch for cloud detection, demonstrating that it can be deployed without further adaptation. For flood detection, however, the pretrained encoder alone underperformed relative to training from scratch; pairing it with a pretrained task head restored performance to match or exceed the baseline. Task head pretraining was therefore not strictly necessary for effective adaptation, but it consistently provided small, measurable gains, and in some cases (e.g., flood detection) was required to achieve parity with models trained from scratch.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Bandwidth-efficient domain adaptation matches full fine-tuning}\label{results2}
% \hl{MAY REMOVE IT DEPENDING ON RESULTS OF 2.2. MENTION THIS IN DISCUSSION SECTION} \\

% \hl{Only use Prithvi-EO-2.0-256-MAE-D here and vary the percentage of weights to update on target domain data. We selected cloud and flood detection as representative tasks since ground truth annotations for the remaining downstream tasks were unavailable}

% \begin{figure}[H]
% \centering
% \begin{subfigure}[b]{0.47\linewidth}
%     % \includegraphics[width=\linewidth]{Figures/cloud-classification-kanyini-sparse.pdf}
%     \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}} % Placeholder box
%     \caption{Cloud detection (tile-level classification)}
%     \label{fig:cloud-classification}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.47\linewidth}
%     % \includegraphics[width=\linewidth]{Figures/cloud-segmentation-kanyini-sparse.pdf}
%     \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}} % Placeholder box
%     \caption{Cloud detection (segmentation)}
%     \label{fig:cloud-segmentation}
% \end{subfigure}

% \vspace{0.5cm}

% \begin{subfigure}[b]{0.47\linewidth}
%     % \includegraphics[width=\linewidth]{Figures/flood-kanyini-sparse.pdf}
%     \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}} % Placeholder box
%     \caption{Flood detection (segmentation)}
%     \label{fig:flood-detection}
% \end{subfigure}
% \hfill
% \caption{Performance of the \texttt{Prithvi} encoder and task heads for cloud and flood detection on Kanyini data. All task head weights are updated during adaptation, as their small size remains within uplink bandwidth constraints. To reduce uplink cost for the larger encoder, only a varying percentage of its weights are updated, simulating bandwidth-efficient domain adaptation. \hl{x-axis - percentage of weights updated, y-axis - model performance}}
% \label{fig:domain-adaptation-results}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Hardware emulator accelerates desgin-test cycle and reproduces flight hardware performance}\label{results3}
% To accelerate development and minimise integration risk, we first evaluated the Prithvi encoder and its associated task heads on a hardware emulator that closely mirrors the compute environment of Kanyini’s HyperScout-2 payload. The emulator consists of a Ubotica CogniSAT-XE1, featuring the Intel Myriad 2 VPU, connected via USB to an Advantech ARK-1123 embedded system, selected for its comparable CPU and memory specifications to the satellite’s onboard data handling unit. This emulated platform provided a flexible and accessible environment for evaluating model performance and debugging software prior to hardware integration. The same software stack, including the runtime environment and ML inference workflows, was deployed across both the emulator and the HyperScout-2 engineering model. Following successful evaluation on the emulator, we repeated the evaluation on the engineering model to confirm deployment readiness under flight-representative conditions. \\

% \begin{table*}[ht]
% \centering
% \small
% \caption{Performance across three tasks on the Kanyini test sets. 
% All metrics are reported as percentages.}
% \label{tab:kanyini-performance}

% % ---------- (a) Cloud classification ----------
% \begin{subtable}{\linewidth}
% \centering
% \small
% \label{tab:cloud_classification_combined}
% \begin{tabular}{l c c c c c}
% \toprule
% \textbf{Environment} & \textbf{\shortstack{Hardware \\ Accelerator}} & \textbf{\shortstack{FP \\ Format}}
% & \textbf{Acc} & \textbf{FP} & \textbf{F1} \\
% \midrule
% \rowcolor{gray!15}\multicolumn{6}{c}{\textbf{Cloud detection  tile-based classification (792 tiles)}}\\
% Workstation       & GPU            & FP32 & 97.22 & 0.76 & 95.22 \\
% Hardware emulator & XE1 (Myriad 2) & FP16 & 97.10 & 0.88 & 95.01 \\
% Engineering model & EoT (Myriad 2) & FP16 & 97.10 & 0.88 & 95.01 \\
% \bottomrule
% \end{tabular}
% \end{subtable}

% \vspace{0.75em}

% % ---------- (b) Cloud segmentation ----------
% \begin{subtable}{\linewidth}
% \centering
% \small
% \label{tab:cloud_segmentation_combined}
% \begin{tabular}{l c c c c c c}
% \toprule
% \textbf{Environment} & \textbf{\shortstack{Hardware \\ Accelerator}} & \textbf{\shortstack{FP \\ Format}}
% & \textbf{mIoU} & \textbf{mF1} & \textbf{OA} & \textbf{FP} \\
% \midrule
% \rowcolor{gray!15}\multicolumn{7}{c}{\textbf{Cloud detection - segmentation (792 tiles)}}\\
% Workstation       & GPU            & FP32 & 90.14 & 94.80 & 95.18 & 1.50 \\
% Hardware emulator & XE1 (Myriad 2) & FP16 & 90.12 & 94.79 & 95.17 & 1.52 \\
% Engineering model & EoT (Myriad 2) & FP16 & 90.12 & 94.79 & 95.17 & 1.52 \\
% \bottomrule
% \end{tabular}
% \end{subtable}

% \vspace{0.75em}

% % ---------- (c) Flood segmentation ----------
% \begin{subtable}{\linewidth}
% \centering
% \small
% \label{tab:flood_segmentation_combined}
% \begin{tabular}{l c c c c c c}
% \toprule
% \textbf{Environment} & \textbf{\shortstack{Hardware \\ Accelerator}} & \textbf{\shortstack{FP \\ Format}}
% & \textbf{mIoU} & \textbf{mF1} & \multicolumn{2}{c}{\textbf{Water}} \\
% \cmidrule(lr){6-7}
%  &  &  &  &  & \textbf{IoU} & \textbf{F1} \\
% \midrule
% \rowcolor{gray!15}\multicolumn{7}{c}{\textbf{Flood detection - segmentation (880 tiles)}}\\
% Workstation       & GPU            & FP32 & 91.45 & 95.46 & 86.49 & 92.76 \\
% Hardware emulator & XE1 (Myriad 2) & FP16 & 91.56 & 95.53 & 86.64 & 92.84 \\
% Engineering model & EoT (Myriad 2) & FP16 & 91.56 & 95.53 & 86.64 & 92.84 \\
% \bottomrule
% \end{tabular}
% \end{subtable}

% \end{table*}

% \hl{ADD QUALITATIVE RESULTS - datacube with tile grid and predicted outputs vs ground truth \\}


% As shown in Table~\ref{tab:kanyini-performance}, reducing numerical precision from single-precision floating point (FP32, 32-bit) to half-precision floating point (FP16, 16-bit), as required by the Myriad-2 VPU, yields only negligible changes in predictive performance across the three EO tasks. For example, cloud classification accuracy is 97.22\% (FP32) versus 97.10\% (FP16), and flood segmentation mIoU differs by only 0.11 percentage points. Similar patterns hold for mF1, OA, false-positive rate, and water-class IoU/F1, with deltas consistently $\leq$\,0.21 percentage points. Notably, the hardware emulator and the engineering model (both FP16 on Myriad-2) produce indistinguishable results at the reported precision, validating the hardware emulator as a faithful proxy for on-board execution. Beyond predictive performance, the emulator enables a 3–4$\times$ faster iteration cycle, substantially accelerating the design–test loop. \\

% Table~\ref{tab:kanyini-efficiency} reports efficiency and resource utilisation per data cube (88 tiles). Inference time per tile is effectively identical across both platforms (e.g., 5.36\,s vs.\ 5.35\,s for cloud classification), runtime differences are small (typically $\leq$\,25\,s per cube), and memory usage is stable at $\sim$630–640\,MB. The primary divergence is in power: peak and average power are systematically higher on the engineering model (e.g., 7.26\,W vs.\ 5.76\,W peak for cloud classification), resulting in slightly higher energy consumption (0.98–1.07\,Wh vs.\ 0.72–0.79\,Wh). Thus, while the emulator provides a rapid, low-power environment for iteration, the engineering model captures the true power envelope of flight hardware, ensuring accurate energy budgeting for on-orbit operations.

% \begin{table*}[ht]
% \centering
% \small
% \caption{Efficiency and resource utilisation per Kanyini data cube (88 tiles).}
% \label{tab:kanyini-efficiency}
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{l c c c c c c}
% \toprule
% \textbf{Environment} 
% & \textbf{\shortstack{Inf time \\ (per tile)}} 
% & \textbf{Runtime} 
% & \textbf{Memory} 
% & \textbf{\shortstack{Peak \\ Power}} 
% & \textbf{\shortstack{Avg \\ Power}} 
% & \textbf{Energy} \\
% & (s) & (s) & (MB) & (W) & (W) & (Wh) \\
% \midrule

% \rowcolor{gray!15}\multicolumn{7}{c}{\textbf{Cloud detection - tile-based classification}} \\
% Hardware emulator & 5.36 & 526.41 & 636.25 & 5.76 & 4.95 & 0.72 \\
% Engineering model & 5.35 & 551.66 & 633.58 & \textbf{7.26} & \textbf{6.41} & 0.98 \\
% \midrule

% \rowcolor{gray!15}\multicolumn{7}{c}{\textbf{Cloud detection - segmentation}} \\
% Hardware emulator & 5.50 & 553.21 & 633.45 & 5.77 & 4.94 & 0.76 \\
% Engineering model & 5.49 & 575.34 & 636.09 & \textbf{7.16} & \textbf{6.39} & 1.02 \\
% \midrule

% \rowcolor{gray!15}\multicolumn{7}{c}{\textbf{Flood detection - segmentation}} \\
% Hardware emulator & 5.68 & 573.42 & 638.18 & 6.20 & 4.97 & 0.79 \\
% Engineering model & 5.67 & 597.43 & 631.77 & \textbf{7.21} & \textbf{6.45} & 1.07 \\
% \bottomrule
% \end{tabular}
% \end{table*}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUPP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[H]
% \centering

% \begin{subfigure}[b]{0.9\linewidth}
%     \vspace{-0.2cm}
%     \includegraphics[width=\linewidth]{Figures/cloud-classification.pdf}
%     \vspace{-1.0cm}
%     \caption{Cloud detection - tile-level classification}
%     \vspace{-0.2cm}
%     \label{fig:cloud-classification}
% \end{subfigure}
% \vspace{-0.2cm}
% \begin{subfigure}[b]{0.9\linewidth}
%     \includegraphics[width=\linewidth]{Figures/cloud-segmentation.pdf}
%     \vspace{-1.0cm}
%     \caption{Cloud detection - segmentation}
%     \label{fig:cloud-segmentation}
% \end{subfigure}
% \vspace{-0.2cm}
% \begin{subfigure}[b]{0.9\linewidth}
%     \includegraphics[width=\linewidth]{Figures/flood.pdf}
%     \vspace{-1.1cm}
%     \caption{Flood detection - segmentation}
%     \label{fig:flood-detection}
% \end{subfigure}
% \vspace{-0.2cm}
% \begin{subfigure}[b]{0.9\linewidth}
%     \includegraphics[width=\linewidth]{Figures/landslide.pdf}
%     \vspace{-1.1cm}
%     \caption{Landslide detection - segmentation}
%     \label{fig:landslide-detection}
% \end{subfigure}
% \vspace{-0.2cm}
% \begin{subfigure}[b]{0.9\linewidth}
%     % \includegraphics[width=\linewidth]{Figures/landcover.pdf}
%     \includegraphics[width=\linewidth]{Figures/cloud-segmentation.pdf} % placeholder
%     \vspace{-1.0cm}
%     \caption{\hl{Land cover classification - segmentation (placeholder)}}
%     \label{fig:flood-detection}
% \end{subfigure}
% \vspace{-0.2cm}
% \begin{subfigure}[b]{0.9\linewidth}
%     \includegraphics[width=\linewidth]{Figures/agb.pdf}
%     % \caption{Above-ground biomass estimation (regression)}
%     \vspace{-1.0cm}
%     \caption{AGB estimation - regression}
%     \label{fig:landslide-detection}
% \end{subfigure}

% \caption{Performance comparison across multiple EO tasks.}
% \label{fig:eo-task-results}
% \end{figure}
